Constraint-Aware Refinement for Safety Verification of Neural Feedback Loops

Neural networks (NNs) are becoming increasingly popular in the design of control pipelines for autonomous systems. However, since the performance of NNs can degrade in the presence of out-of-distribution data or adversarial attacks, systems that have NNs in their control pipelines, i.e., neural feedback loops (NFLs), need safety assurances before they can be applied in safety-critical situations. Reachability analysis offers a solution to this problem by calculating reachable sets that bound the possible future states of an NFL and can be checked against dangerous regions of the state space to verify that the system does not violate safety constraints. Since exact reachable sets are generally intractable to calculate, reachable set over approximations (RSOAs) are typically used. The problem with RSOAs is that they can be overly conservative, making it difficult to verify the satisfaction of safety constraints, especially over long time horizons or for highly nonlinear NN control policies. Refinement strategies such as partitioning or symbolic propagation are typically used to limit the conservativeness of RSOAs, but these approaches come with a high computational cost and often can only be used to verify safety for simple reachability problems. This paper presents Constraint-Aware Refinement for Verification (CARV): an efficient refinement strategy that reduces the conservativeness of RSOAs by explicitly using the safety constraints on the NFL to refine RSOAs only where necessary. We demonstrate that CARV can verify the safety of an NFL where other approaches either fail or take up to 60x longer and 40x the memory.

==> numerical_results.tex <==
%!TEX root=main.tex

\section{Numerical Results}
\label{sec:results}
This section presents results from numerical experiments that demonstrate the properties of CARV.
We compare CARV to three existing refinement approaches: partitioning~\cite{everett2021reachability} (\meth{part}), pure symbolic propagation~\cite{chen2023one} (\meth{symb}), and hybrid-symbolic propagation~\cite{sidrane2022overt} (\meth{hybr}).
We show that CARV outperforms existing methods for a relatively simple double integrator example, as well as a more complicated ground robot example that requires safety verification over 52 time steps.
Reachable sets are generated with the AutoLiRPA CG analysis tool~\cite{xu2020automatic} using CROWN~\cite{zhang2018efficient} to generate bounds.
All experiments were conducted on a machine running Ubuntu 22.04 with an i7-6700K CPU and 32 GB of RAM.


\subsection{Double Integrator}
\label{sec:results:double_integrator}

First, we demonstrate CARV's behavior on a double integrator model
\begin{equation}
    \label{eqn:di_dynamics}
    \mathbf{x}_{t+1} =
    \begin{bmatrix}
    1 & dt \\
    0 & 1
    \end{bmatrix} \mathbf{x}_t +
    \begin{bmatrix}
    \frac{1}{2} dt^2 \\ dt
    \end{bmatrix} \mathbf{u}_t
\end{equation}
with $dt = 0.2$ and where $\you_t = \picl(\x_t)$ has 3 hidden layers with [30, 20, 10] neurons, ReLU activations, and was trained using an MPC expert to drive the state to ${\x = [0, 0]^\top}$ while satisfying the constraints
\begin{equation}
    \label{eqn:di_constraints}
    c(\x) = (\x[0] \geq 0\ \mathrm{and}\ \x[1] \geq -1),
\end{equation}
where $\x[0]$ and $\x[1]$ are the first and second states, respectively.
We denote the problem defined above as \exper{DI}.

\cref{fig:double_integrator} shows how CARV is able to verify safety against the constraints \cref{eqn:di_constraints} (gray) over ${t_f = 30}$ time steps with ${k_{max} = 15}$.
Monte Carlo samples (black markers) are propagated from the initial state set (black rectangle) as a proxy for the true behavior of the system.
In \cref{fig:double_integrator:conflict}, concrete RSOAs (blue) are calculated until $\rsoa{5}$ (orange) (calculated from $\rsoa{4}$, magenta) violates $c$.
\cref{fig:double_integrator:resolved} shows the result of calling $\mathtt{refine}$ on $\rsoa{5}$ in \cref{fig:double_integrator:conflict}: $\rsoa{5}$ (green) is refined as a symbolic RSOA from $\rsoa{0}$ (magenta).
\cref{fig:double_integrator:final} shows the result of iterating the processes shown in \cref{fig:double_integrator:conflict} and \cref{fig:double_integrator:resolved}: safety is successfully verified.
The example in \cref{fig:double_integrator} was calculated in \SI{3.71}{s}.


% \begin{figure*}[ht!]
%     \centering
%     % \captionsetup[subfigure]{aboveskip=-4pt,belowskip=-4pt}
%     \begin{subfigure}[t]{0.325\textwidth}
%         \centering
%         \captionsetup{width=.9\columnwidth}
%         \includegraphics[width=1\columnwidth,trim={0 0 0 0},clip]{figures/double_integrator/double_integrator_CARV_conflict.png}
%         \caption{Concrete RSOAs (blue) are calculated until $\rsoa{5}$ (orange) calculated from $\rsoa{4}$ (magenta) violates the safety constraint (gray).}
%         \label{fig:double_integrator:conflict}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.325\textwidth}
%         \centering
%         \captionsetup{width=.9\columnwidth}
%         \includegraphics[width=1\columnwidth,trim={0 0 0 0},clip]{figures/double_integrator/double_integrator_CARV_resolved.png}
%         \caption{CARV uses $\mathtt{refine}$ (\cref{alg:refine}) to deconflict $\rsoa{5}$ with the constraint ${\x[0] \geq -1}$.
%         The refined RSOA (green) is the result of a symbolic reachability calculation from $\rsoa{0}$ (magenta).}
%         \label{fig:double_integrator:resolved}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.325\textwidth}
%         \centering
%         \captionsetup{width=.9\columnwidth}
%         \includegraphics[width=1\columnwidth,trim={0 0 0 0},clip]{figures/double_integrator/double_integrator_CARV_final.png}
%         \caption{
%         CARV calculates concrete RSOAs (blue) which can be very conservative unless they violate the contraints (gray), in which case the RSOA is refined with a symbolic calculation (green).
%         }
%         \label{fig:double_integrator:final}
%     \end{subfigure}
%     \caption{Successive frames of CARV's solution to \exper{DI} showing how CARV detects a collision (\cref{fig:double_integrator:conflict}), fixes it with refinement (\cref{fig:double_integrator:resolved}), and repeats until the problem is successfully verified (\cref{fig:double_integrator:final}).}
%     \label{fig:double_integrator}
% \end{figure*}







% \begin{figure}[t]
%     \centering
%     % \captionsetup[subfigure]{aboveskip=-4pt,belowskip=-4pt}
%     \begin{subfigure}{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth,trim={0 0 0 0},clip]{figures/double_integrator/double_integrator_CARV_conflict.png}
%         \caption{Caption}
%         \label{fig:enter-label}
%     \end{subfigure}
%     \begin{subfigure}{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth,trim={0 0 0 0},clip]{figures/double_integrator/double_integrator_CARV_resolved.png}
%         \caption{Caption}
%         \label{fig:enter-label}
%     \end{subfigure}
%     \begin{subfigure}{\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth,trim={0 0 0 0},clip]{figures/double_integrator/double_integrator_CARV_final.png}
%         \caption{Caption}
%         \label{fig:enter-label}
%     \end{subfigure}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}


\subsection{Ground Robot}
\label{sec:results:ground_robot}

Next, we compare CARV to existing techniques with a verification problem for a ground robot with nonlinear dynamics
\begin{equation}
    \label{eqn:unicycle_dynamics}
    \mathbf{x}_{t+1} =
    \underbrace{
    \begin{bmatrix}
        x_t \\ y_t \\ \psi_t
    \end{bmatrix}}_{\x_t} +
    \begin{bmatrix}
        v\cos(\psi_t) \\ v\sin(\psi_t) \\ \omega_t
    \end{bmatrix} dt,
\end{equation}
where $(x_t,\ y_t)$ is the position of the robot, $\psi_t$ is it's heading, $v = 1$ is constant, $\omega_t$ is the input, and $dt = 0.2$.
The input $\omega_t$ is the output of a NN, i.e., $\omega_t = \picl(\x)$, where $\picl$ has 3 hidden layers with [40, 20, 10] neurons, ReLU activations, and was trained using an MPC expert to drive the position to ${(x, y) = (0, 0)}$ while avoiding two circular obstacles, i.e., satisfying the constraints
\begin{equation}
    \label{eqn:unicycle_constraints}
    \begin{split}c(\x) =  (
        & (x - c_{x1})^2 + (y - c_{y1})^2 \geq r_1^2 \ \mathrm{and} \\ & (x - c_{x2})^2 + (y - c_{y2})^2 \geq r_2^2)),
        \end{split}
\end{equation}
where $(c_{x1},\ c_{y1},\ r_1) = (-6,\ -0.5,\ 2.2)$ and $(c_{x2},\ c_{y2},\ r_2) = (-1.25,\ 1.75,\ 1.6)$ represent the $x-y$ positions and radii of the first and second obstacles, respectively.
We denote the problem above as \exper{GR} and show the corresponding outputs from \meth{part} (\cref{fig:ground_robot:part}), \meth{symb},
\meth{hybr} (\cref{fig:ground_robot:TTT}), and CARV (\cref{fig:ground_robot:CARV}) in \cref{fig:ground_robot}.
% We selected a maximum symbolic horizon $k_{max} = 10$ for both \meth{hybr} and CARV.

Partitioning (\meth{part}) is an approach where the initial state set is split into smaller subsets.
By doing RSOA calculations for each of the subsets, the CG relaxations $\lFcl{}$ and $\uFcl{}$ are taken over smaller regions and can thus be tighter.
As shown in \cref{fig:ground_robot:part}, this strategy can be used to verify \exper{GR} as safe.
The main problem with \meth{part} is that it scales poorly with the dimension of the state space.
In order to verify safety for \exper{GR} using \meth{part}, the initial state set had to be split into $6\times6\times18$ uniform partitions.
Since \exper{GR} needs to be verified over 52 time steps, this means \meth{part} makes 33696 concrete RSOA calculations, which takes \SI{516}{s} and uses all 32 GB of available RAM.
An additional challenge associated with \meth{part} is that an effective partitioning scheme is nontrivial to find.
While guided partitioning strategies exist \cite{everett2020robustness}, these approaches can take many iterations to converge, so we used trial and error to find a uniform partitioning configuration that worked.

Pure symbolic propagation (\meth{symb}) is another approach that can work well for small problems.
However, as noted in \cref{fig:ground_robot:part}, it is intractable to use over long time horizons.
In the case of \exper{GR}, the nonlinearites in the system and NN controller make for a challenging problem to calculate symbolically for many steps, causing \meth{symb} to reach our set time limit of 30 minutes (\SI{1800}{s}), at which point it had calculated 19 RSOAs.
% Extrapolating the computation time from the first 19 steps to the entire horizon indicates \meth{symb} would take approximately 24000 years to verify \exper{GR} as safe.
% The theoretical computational complexity of CROWN scales in polynomial time with respect to the number of layers in the NN being analyzed, 

Hybrid-symbolic propagation (\meth{hybr}) was introduced in \cite{sidrane2022overt} and recently employed as the refinement strategy for \cite{sidrane2024ttt}.
In hybrid symbolic propagation, symbolic RSOAs are calculated from previous symbolic RSOAs on a given schedule, with concrete RSOAs filling in the gaps.
While significant effort could be expended to find a hybrid schedule that works for a specific problem, we will consider a uniform schedule that makes symbolic calculations every $k_{max} = 10$ steps.
\cref{fig:ground_robot:TTT} shows the result produced by \meth{hybr} for \exper{GR}, which was calculated in \SI{16}{s}.
While much faster than \meth{part} and \meth{symb}, two RSOAs toward the end (orange) intersect with the obstacle, meaning that \meth{hybr} cannot verify \exper{GR} as safe in this configuration.
In \cref{sec:results:k_max} we investigate the importance of $k_{max}$ on this outcome.

Finally, the result of using CARV with $k_{max} = 10$ on \exper{GR} is shown in \cref{fig:ground_robot:CARV}.
Since none of the RSOAs in the final result intersect with the obstacle, CARV verifies that \exper{GR} is safe.
Moreover, it takes \SI{13}{s} to run, thereby also outperforming existing methods in calculation time.
Notice that similar to \meth{hybr}, CARV calculates symbolic RSOAs at $k_{max}$ intervals.
However, CARV only does this \emph{as needed} to save on time, and in fact, for \exper{GR}, calculates only concrete RSOAs up to $t=35$ before there is a conflict with the second obstacle, triggering a call to $\mathtt{refine\_sequence}$ that refines RSOAs at $k_{max}$ intervals tracing back to $\mathcal{X}_0$.
% Another key feature of CARV is that it also does symbolic calculations on \emph{shorter} intervals than $k_{max}$ as needed.
% This is ultimately what allows CARV to verify \exper{GR} as safe whereas \meth{hybr} fails due to the wrapping effect influencing the concrete RSOAs between symbolic calculations.
The results from each refinement method for \exper{GR} and \exper{DI} are summarized in \cref{tab:alg_comparison}.

\begin{figure}[ht!]
    \centering
    % \captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
    \begin{subfigure}{0.97\columnwidth}
        \centering
        \includegraphics[width=1\columnwidth,trim={25 10 36 25pt},clip]{figures/ground_robot/unicycle_part_final_r1.pdf}
        \caption{\meth{part} calculates partitioned concrete RSOAs (blue) to verify \exper{GR} as safe in \SI{516}{s} and uses 32 GB of RAM. 
        \meth{symb} calculates 19 symbolic RSOAs then times out at 1800 seconds.}
        \label{fig:ground_robot:part}
    \end{subfigure}
    % \begin{subfigure}{0.97\columnwidth}
    %     \centering
    %     \includegraphics[width=1\columnwidth,trim={0cm 0cm 2cm 1cm},clip]{figures/ground_robot/unicycle_symb_final.png}
    %     \caption{\meth{symb} calculates 19 symbolic RSOAs (green), then times out at 1800 seconds.}
    %     \label{fig:ground_robot:symb}
    % \end{subfigure}
    \begin{subfigure}{0.97\columnwidth}
        \centering
        \includegraphics[width=1\columnwidth,trim={25 10 36 25pt},clip]{figures/ground_robot/unicycle_hybr_final_r1.pdf}
        \caption{\meth{hybr} produces RSOAs (orange) that violate the safety constraints, and is thus unable to verify \exper{GR} as safe.}
        \label{fig:ground_robot:TTT}
    \end{subfigure}
    \begin{subfigure}{0.97\columnwidth}
        \centering
        \includegraphics[width=1\columnwidth,trim={25 10 36 25pt},clip]{figures/ground_robot/unicycle_CARV_final_r1.pdf}
        \caption{CARV verifies \exper{GR} as safe in \SI{13}{s} of computation time using a combination of concrete (blue) and refined (green) RSOAs.}
        \label{fig:ground_robot:CARV}
    \end{subfigure}
    \caption{CARV (ours) outperforms \meth{part}, \meth{symb}, and \meth{hybr} in computation time and ability to verify safety for \exper{GR}.}
    \label{fig:ground_robot}
    \vspace{-12pt}
\end{figure}

\begin{table}[t]
    \centering
    \caption{CARV efficiently verifies safety for \exper{DI} and \exper{GR}. $^{\bm{*}}$indicates verification unsuccessful.}

    \normalsize
    \begin{tabular}{lcc}
        \hline
        Approach & \exper{DI} [s] & \exper{GR} [s] \\
        \hline
        \meth{part} \cite{everett2021reachability} & $18.81 \pm 0.82$ & $516.48 \pm 5.68$ \\
        \meth{symb} \cite{chen2023one} & $25.82 \pm 0.50$ & timed out (\SI{1800}{s}) \\
        \meth{hybr} \cite{sidrane2022overt} & $1.60^{\bm{*}} \pm 0.07$ & $15.75^{\bm{*}} \pm 0.56$ \\
        CARV (\textbf{ours}) & $\mathbf{3.71 \pm 0.16}$ & $\mathbf{13.11 \pm 0.47}$ \\
        \hline
    \end{tabular}
    \vspace{-16pt}
    \label{tab:alg_comparison}
\end{table}





\subsection{Varying the Maximum Symbolic Horizon}
\label{sec:results:k_max}
Next we investigate CARV's sensitivity to the hyperparameter $k_{max}$ when applied to \exper{GR}.
\cref{fig:ground_robot_comparison} shows results from both \meth{hybr} and CARV given $k_{max}$ values ranging from 6 to 14.
For $k_{max} < 8$, symbolic calculations are short and frequent so neither \meth{hybr} or CARV can sufficiently reduce the wrapping effect, thus leading to a failure to verify \exper{GR} as safe.
At $k_{max} = 8$, both \meth{hybr} and CARV verify \exper{GR} as safe, but for all tested $k_{max} > 8$, \meth{hybr} fails to verify \exper{GR} as safe whereas CARV verifies safety in each case.
% We also note that for $k_{max}=8$, \meth{hybr} is very close to failing -- a 1\% increase in the radius of the second obstacle is enough to cause a violation of the safety constraints.
% The trends shown in \cref{fig:ground_robot_comparison:time} illustrate the differences in design objectives between \meth{hybr} and CARV.
% For \meth{hybr}, increasing $k_{max}$ equates to increasing the time budget, thus leading to a monotonic increase in computation time.
Notice CARV spends more time in the cases where verification fails ($k_{max} = 6,\ 7$) because it tries to refine as much as possible in an attempt to verify safety.
Moreover, because CARV only refines RSOAs as needed and prioritizes symbolic calculations shorter than $k_{max}$, it is faster than \meth{hybr} when $k_{max}$ is large. 
% \cref{fig:ground_robot_comparison:error} shows another useful property of CARV in that its result tends to converge to a maximum safe approximation error \cite{sidrane2024ttt}, defined as
% \begin{equation*}
%     \mathrm{approximation \ error} = \frac{\sum_{i=1}^{t_f}\mathrm{volume}(\rsoa{i})}{\sum_{i=1}^{t_f}\mathrm{volume}(\ubar{\mathcal{R}}_{i})},
% \end{equation*}
% where $\ubar{\mathcal{R}}_{i}$ is a hyper-rectangular under-approximation of the true reachable set at time $i$, calulated using Monte Carlo sampling. 
% The trend produced by CARV is in contrast to \meth{}, where the wrapping effect compounds from symbolic RSOA to symbolic RSOA when $k_{max}$ is small, and compounds in the concrete RSOAs between the symbolic RSOAs when $k_{max}$ is large.    


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/ground_robot/comparison_time.png}
%     \caption{}
%     \label{fig:ground_robot_comparison}
% \end{figure}

\begin{figure}[t]
    \centering
    % \captionsetup[subfigure]{aboveskip=-2pt,belowskip=-2pt}
    \includegraphics[width=0.8\columnwidth,trim={20pt 24pt 42pt 36pt},clip]{figures/ground_robot/comparison_time_r4.png}
    \caption{CARV verifies \exper{GR} as safe for all tested $k_{max} \geq 8$.}
    % \vspace{-12pt}
    \label{fig:ground_robot_comparison}
%\end{figure}
%\begin{figure}[t]
    \centering
    % \captionsetup[subfigure]{aboveskip=-2pt,belowskip=-2pt}
    \hspace*{12pt}\includegraphics[width=0.85\columnwidth,trim={20pt 24pt 12pt 36pt},clip]{figures/tighten_constraints/sweep_unicycle_constraint_r4.png}
    \vspace{-3pt}
    \caption{CARV can verify harder problems than \meth{hybr} or \meth{part}. Dashed vertical lines mark largest values of $\Delta r$ that can be verified by each algorithm.}
    \vspace{-12pt}
    \label{fig:sweep_constraint}
\end{figure}


\subsection{Verification Analysis}
Finally, we investigate CARV's ability to verify more challenging problems by introducing the parameter $\Delta r$ and solving a series of problems \experc{GR}{\Delta r} with the same constraint function \cref{eqn:unicycle_constraints} as \exper{GR}, but with radii $r_1 + \Delta r$ and $r_2 + \Delta r$.
As the radii of the two obstacles increase, the RSOAs must become less conservative to successfully verify safety, thus making the problem more difficult.
\cref{fig:sweep_constraint} shows successful verifications from CARV, \meth{part}, and \meth{hybr} on different \experc{GR}{\Delta r} where $\Delta r \in [0, 0.26]$.
The dashed vertical lines mark the largest values of $\Delta r$ that can be verified by each algorithm.
We set $k_{max} = 8$ for \meth{hybr} (magenta) since that was the only value that verified \exper{GR}  (\cref{fig:ground_robot_comparison}), but \meth{hybr} fails with $\Delta r = 0.002$.
Since \meth{part} (orange) uses all available RAM to verify \exper{GR}, we use the same partitioning scheme as in \cref{sec:results:ground_robot}, which verifies each \experc{GR}{\Delta r} with $\Delta r \leq 0.11$.
CARV is tested with $k_{max}$ values 10 and 14, denoted $\mathrm{CARV}_{10}$ (blue) and $\mathrm{CARV}_{14}$ (green), respectively.
Unlike \meth{part} and \meth{hybr}, CARV adjusts to the difficulty of the problem and thus has lower calculation times for lower values of $\Delta r$.
Additionally, CARV verifies more difficult problems than \meth{part} or \meth{hybr} -- we achieve verification up to \experc{GR}{0.20} and \experc{GR}{0.26} with $\mathrm{CARV}_{10}$ and $\mathrm{CARV}_{14}$, respectively.
Note that for hyper-rectangular RSOAs, $\Delta r = 0.33$ is the highest verifiable value.



